MUTANT: A Multi-sentential Code-mixed Hinglish Dataset

The multi-sentential long sequence textual data unfolds several interesting research directions pertaining to natural language processing and generation. Though we observe several high-quality long-sequence datasets for English and other monolingual languages, there is no significant effort in building such resources for code-mixed languages such as Hinglish (code-mixing of Hindi-English). In this paper, we propose a novel task of identifying multi-sentential code-mixed text (MCT) from multilingual articles. As a use case, we leverage multilingual articles from two different data sources and build a first-of-its-kind multi-sentential code-mixed Hinglish dataset i.e., MUTANT. We propose a token-level language-aware pipeline and extend the existing metrics measuring the degree of code-mixing to a multi-sentential framework and automatically identify MCT in the multilingual articles. The MUTANT dataset comprises 67k articles with 85k identified Hinglish MCTs. To facilitate future research, we make the publicly available.

==> figures/MUTANT_arch.tex <==
\begin{figure}[]
    \centering
    \includegraphics[width=0.2\linewidth]{EMNLP 2022/figures/MUTANT_arch.pdf}
    \caption{Architecture of MCT identification pipeline.}
    \label{fig: arch}
\end{figure}

==> figures/cm_example.tex <==
\begin{figure}[]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/example.png}
    \caption{Example news article from Dainik Jagran website containing a Hinglish paragraph. An article in \textit{LongCoMix} dataset can have multiple Hinglish paragraphs. In the example, we color code the text containing \textcolor{orange}{Hindi} and \textcolor{blue}{English} tokens. The language independent tokens are marked with black color. \textcolor{red}{@RG: can you add one example paragraph from political speeches as well?}}
    \label{fig: cm_example}
\end{figure}

==> figures/false_positive.tex <==
\begin{figure}[t]
\centering
\small{
\begin{tcolorbox}[colback=white]

\begin{center}
    \textbf{\underline{Example I}}
    \\
\end{center}

\bigbreak
...\begin{hindi}\textcolor{orange} {मैं आप सभी को}, \textcolor{orange}{इस विचार को साकार करने वाली पूरी} \textcolor{blue}{टीम} \textcolor{orange}{को शुभकामनाएँ देता हूँ}। \textcolor{orange}{जैसे भी हमारे} \textcolor{blue}{ स्पीकर} \textcolor{orange}{साहब ने बताया}, \textcolor{orange}{आज } दूरदर्शन \textcolor{orange}{ की स्थापना के भी }62 \textcolor{orange}{ वर्ष पूरे हुए हैं}। \textcolor{orange}{ये बहुत लंबी यात्रा है}। \textcolor{orange}{इस यात्रा को सफल बनाने में अनेकों लोगों का योगदान रहा है}। \textcolor{orange}{मैं} दूरदर्शन \textcolor{orange}{ के संचालन से जुड़े सभी लोगों को भी बधाई देता हूं}।\end{hindi}...

\begin{center}
    \textbf{\underline{Example II}}
    \\
\end{center}
\bigbreak

...\begin{hindi}\textcolor{orange}{आज जब देश अपनी आज़ादी के} 75 \textcolor{orange}{साल मना रहा है}, \textcolor{orange}{तो हमारे सामने अतीत का गौरव भी है और भविष्य के संकल्प भी हैं}। \textcolor{orange}{इन दोनों ही क्षेत्रों में} \textcolor{blue}{मीडिया} \textcolor{orange}{की बहुत बड़ी भूमिका है}। \textcolor{blue}{मीडिया} \textcolor{orange}{जब किसी विषय को उठाता है}, \textcolor{orange}{जैसे स्वच्छ भारत अभियान}, \textcolor{orange}{तो वो और तेजी से जन-जन तक पहुंचाता है}। \textcolor{orange}{आज़ादी के अमृत महोत्सव में देशवासियों के प्रयासों को प्रचारित-प्रसारित करने का कार्य} \textcolor{blue}{मीडिया} \textcolor{orange}{बखूबी कर सकता है}। \textcolor{orange}{उदाहरण के तौर पर}, \textcolor{blue}{टीवी चैनल्स} \textcolor{orange}{स्वतन्त्रता संग्राम से जुड़े} 75 \textcolor{blue}{एपिसोड्स प्लान} \textcolor{orange}{कर सकते हैं}\end{hindi}, \textcolor{blue}{documentaries} \begin{hindi}  \textcolor{orange}{बना सकते हैं}। \textcolor{orange}{अख़बार अमृत महोत्सव से जुड़े परिशिष्ट प्रकाशित कर सकते हैं}। \textcolor{blue}{डिजिटल मीडिया}\end{hindi} \textcolor{blue}{quiz}, \textcolor{blue}{competition} \begin{hindi}  \textcolor{orange}{जैसे} \end{hindi} \textcolor{blue}{ideas} \begin{hindi}        \textcolor{orange}{के जरिए युवाओं को सीधे जोड़ सकते हैं}।\end{hindi}...

\end{tcolorbox}}
\caption{Example \textit{false positives} from the MVT technique where both the paragraphs are identified as code-mixed. In Example I, both the evaluators agree that the paragraph is not code-mixed, whereas in Example II, only one of the evaluators identify the paragraph as code-mixed. We use the same color encoding as in Figure \ref{fig: example} (i.e., \textcolor{orange}{Hindi}, \textcolor{blue}{English}, and language independent).}
\label{fig: false_pos}
\end{figure}

==> figures/pipeline_datacollection.tex <==
\begin{figure*}[]
    \centering
    \includegraphics[width = 16 cm]{figures/pipeline_data_collection.jpeg}
    \caption{Data collection pipeline\textcolor{red}{@RG: is it possible to share the editable source with me? I will try to update this figure} }
    \label{fig:data_collection}
\end{figure*}

==> figures/section_3_2.tex <==
\begin{figure}[t]
\centering
\small{
\begin{tcolorbox}[colback=white]
\begin{center}
    \textbf{\underline{NEWS article heading}}
\end{center}
\bigbreak
\begin{hindi}संयुक्त रूप से संसद टीवी के शुभारम्‍भ अवसर पर प्रधानमंत्री का सम्‍बोधन \end{hindi}

\begin{center}
    \textbf{\underline{NEWS article with a Hinglish paragraph}}
    \\
\end{center}

\bigbreak
...\begin{hindi}आज जब देश अपनी आज़ादी के 75 साल मना रहा है, तो हमारे सामने अतीत का गौरव भी है और भविष्य के संकल्प भी हैं। इन दोनों ही क्षेत्रों में मीडिया की बहुत बड़ी भूमिका है। मीडिया जब किसी विषय को उठाता है, जैसे स्वच्छ भारत अभियान, तो वो और तेजी से जन-जन तक पहुंचाता है। आज़ादी के अमृत महोत्सव में देशवासियों के प्रयासों को प्रचारित-प्रसारित करने का कार्य मीडिया बखूबी कर सकता है। उदाहरण के तौर पर, टीवी चैनल्स स्वतन्त्रता संग्राम से जुड़े 75 एपिसोड्स प्लान कर सकते हैं\end{hindi}, documentaries \begin{hindi}  बना सकते हैं। अख़बार अमृत महोत्सव से जुड़े परिशिष्ट प्रकाशित कर सकते हैं। डिजिटल मीडिया\end{hindi} quiz, competition \begin{hindi}  जैसे \end{hindi} ideas \begin{hindi}  के जरिए युवाओं को सीधे जोड़ सकते हैं।\end{hindi}...
\end{tcolorbox}}
\caption{Only one of the annotators agree that the paragraph is not code-mixed but our model has identified it as the code-mixed paragraph.}
\label{fig:section_3_1}
\end{figure}

==> tables/D_k.tex <==
\begin{table*}[]
\resizebox{\hsize}{!}{
\begin{tabular}{|l|llllllllllllllllllllllllllllll}
\hline
             & \multicolumn{6}{l|}{\textbf{LA}}                                              & \multicolumn{6}{l|}{\textbf{GA}}                                              & \multicolumn{6}{l|}{\textbf{ALG}}                                             & \multicolumn{6}{l|}{\textbf{SDG}}                                             & \multicolumn{6}{l|}{\textbf{MDG}}                                             \\ \hline
             & \multicolumn{3}{l|}{\textbf{D@10}}    & \multicolumn{3}{l|}{\textbf{D@25}}    & \multicolumn{3}{l|}{\textbf{D@10}}    & \multicolumn{3}{l|}{\textbf{D@25}}    & \multicolumn{3}{l|}{\textbf{D@10}}    & \multicolumn{3}{l|}{\textbf{D@25}}    & \multicolumn{3}{l|}{\textbf{D@10}}    & \multicolumn{3}{l|}{\textbf{D@25}}    & \multicolumn{3}{l|}{\textbf{D@10}}    & \multicolumn{3}{l|}{\textbf{D@25}}    \\ \hline
             & \textbf{N} & \textbf{S} & \textbf{NS} & \textbf{N} & \textbf{S} & \textbf{NS} & \textbf{N} & \textbf{S} & \textbf{NS} & \textbf{N} & \textbf{S} & \textbf{NS} & \textbf{N} & \textbf{S} & \textbf{NS} & \textbf{N} & \textbf{S} & \textbf{NS} & \textbf{N} & \textbf{S} & \textbf{NS} & \textbf{N} & \textbf{S} & \textbf{NS} & \textbf{N} & \textbf{S} & \textbf{NS} & \textbf{N} & \textbf{S} & \textbf{NS} \\ \cline{1-1}
\textbf{AAP} & 60         & 49         & 55          & 42         & 23         & 26          & 58         & 46         & 60          & 32         & 24         & 33          & 62         & 51         & 57          & 40         & 24         & 28          & 70         & 60         & 65          & 43         & 41         & 39          & 72         & 62         & 66          & 48         & 25         & 21          \\ \cline{1-1}
\textbf{INC} & 58         & 49         & 57          & 41         & 23         & 27          & 58         & 46         & 60          & 32         & 24         & 33          & 58         & 51         & 56          & 39         & 24         & 29          & 65         & 59         & 62          & 44         & 39         & 37          & 66         & 59         & 63          & 40         & 23         & 21          \\ \cline{1-1}
\textbf{MKB} & 73         & 51         & 62          & 52         & 25         & 32          & 58         & 46         & 60          & 32         & 24         & 33          & 71         & 48         & 65          & 50         & 29         & 34          & 79         & 68         & 68          & 54         & 42         & 42          & 80         & 70         & 65          & 55         & 25         & 24          \\ \cline{1-1}
\textbf{PIB} & 73         & 53         & 63          & 53         & 24         & 33          & 58         & 46         & 60          & 32         & 24         & 33          & 71         & 55         & 64          & 50         & 23         & 34          & 79         & 73         & 75          & 56         & 48         & 52          & 79         & 74         & 74          & 54         & 28         & 28          \\ \cline{1-1}
\textbf{PMS} & 63         & 51         & 57          & 47         & 27         & 27          & 58         & 46         & 60          & 32         & 24         & 33          & 63         & 53         & 59          & 39         & 29         & 29          & 71         & 67         & 65          & 49         & 45         & 44          & 69         & 69         & 69          & 42         & 26         & 23          \\ \cline{1-1}
\textbf{DB}  & 76         & 57         & 64          & 58         & 23         & 30          & 72         & 56         & 62          & 45         & 32         & 34          & 74         & 57         & 62          & 53         & 25         & 34          & 84         & 78         & 76          & 59         & 52         & 50          & 85         & 78         & 75          & 60         & 30         & 29          \\ \cline{1-1}
\textbf{DJ}  & 70         & 48         & 57          & 52         & 21         & 28          & 72         & 56         & 62          & 45         & 32         & 34          & 68         & 49         & 62          & 48         & 24         & 33          & 77         & 73         & 71          & 55         & 50         & 46          & 73         & 74         & 74          & 52         & 31         & 25          \\ \cline{1-1}
\end{tabular}}
\end{table*}

==> tables/accuracy.tex <==
\begin{table}[!tbh]
\centering
\begin{tabular}{l|ccc|ccc}
\hline
\multirow{2}{*}{\textit{Source}} & \multicolumn{3}{c|}{\textit{SDG}}                                          & \multicolumn{3}{c}{\textit{MDG}}  \\
                        & \multicolumn{1}{l}{$A_s$} & \multicolumn{1}{l}{$A_n$} & $A_{s+n}$ & $A_s$ & $A_n$ & $A_{s+n}$ \\ \hline
AAP                     & 72                       & 72                       & 73         & 73   & 74   & 74         \\
MKB                     & 70                       & 69                       & 70         & 72   & 72   & 72         \\
PIB                     & 70                       & 67                       & 67         & 73   & 72   & 73         \\
PMS                     & 74                       & 71                       & 72         & 73   & 74   & 74         \\
INC                     & 73                       & 73                       & 73         & 73   & 74   & 74         \\
DB                      & 68                       & 67                       & 67         & 71   & 78   & 75         \\
DJ                      & 72                       & 75                       & 74         & 71   & 78   & 75  \\ \hline      
\end{tabular}
\caption{}
\label{}
\end{table}

==> tables/parameter_detailed.tex <==
\begin{table*}[]
\resizebox{\hsize}{!}{
\begin{tabular}{|c|ccccc|ccccc|ccccc|ccccc|ccccc|ccccc|}
\hline
\textbf{Category}                       & \multicolumn{5}{c|}{\textbf{E\_s}}                                                                                                                                         & \multicolumn{5}{c|}{\textbf{M\_s}}                                                                                                                                        & \multicolumn{5}{c|}{\textbf{E\_n}}                                                                                                                                         & \multicolumn{5}{c|}{\textbf{M\_n}}                                                                                                                                        & \multicolumn{5}{c|}{\textbf{E\_ns}}                                                                                                                                        & \multicolumn{5}{c|}{\textbf{M\_ns}}                                                                                                                                       \\ \hline
\textbf{}                               & \multicolumn{1}{c|}{\textbf{Prec}} & \multicolumn{1}{c|}{\textbf{Rec}} & \multicolumn{1}{c|}{\textbf{F-s}} & \multicolumn{1}{c|}{\textbf{Acc}} & \textbf{Acc2}             & \multicolumn{1}{c|}{\textbf{Pre}} & \multicolumn{1}{c|}{\textbf{Rec}} & \multicolumn{1}{c|}{\textbf{F-s}} & \multicolumn{1}{c|}{\textbf{Acc}} & \textbf{Acc2}             & \multicolumn{1}{c|}{\textbf{Prec}} & \multicolumn{1}{c|}{\textbf{Rec}} & \multicolumn{1}{c|}{\textbf{F-s}} & \multicolumn{1}{c|}{\textbf{Acc}} & \textbf{Acc2}             & \multicolumn{1}{c|}{\textbf{Pre}} & \multicolumn{1}{c|}{\textbf{Rec}} & \multicolumn{1}{c|}{\textbf{F-s}} & \multicolumn{1}{c|}{\textbf{Acc}} & \textbf{acc2}             & \multicolumn{1}{c|}{\textbf{Prec}} & \multicolumn{1}{c|}{\textbf{Rec}} & \multicolumn{1}{c|}{\textbf{F-s}} & \multicolumn{1}{c|}{\textbf{Acc}} & \textbf{Acc2}             & \multicolumn{1}{c|}{\textbf{Pre}} & \multicolumn{1}{c|}{\textbf{Rec}} & \multicolumn{1}{c|}{\textbf{F-s}} & \multicolumn{1}{c|}{\textbf{Acc}} & \textbf{Acc2}             \\ \hline
\textbf{AAP}                            & \multicolumn{1}{c|}{0.68}          & \multicolumn{1}{c|}{0.65}         & \multicolumn{1}{c|}{0.66}         & \multicolumn{1}{c|}{0.72}         & 0.56                      & \multicolumn{1}{c|}{0.67}         & \multicolumn{1}{c|}{0.63}         & \multicolumn{1}{c|}{0.65}         & \multicolumn{1}{c|}{0.73}         & 0.58                      & \multicolumn{1}{c|}{0.63}          & \multicolumn{1}{c|}{0.63}         & \multicolumn{1}{c|}{0.63}         & \multicolumn{1}{c|}{0.73}         & 0.39                      & \multicolumn{1}{c|}{0.60}         & \multicolumn{1}{c|}{0.59}         & \multicolumn{1}{c|}{0.59}         & \multicolumn{1}{c|}{0.74}         & 0.43                      & \multicolumn{1}{c|}{0.65}          & \multicolumn{1}{c|}{0.63}         & \multicolumn{1}{c|}{0.64}         & \multicolumn{1}{c|}{0.73}         & 0.47                      & \multicolumn{1}{c|}{0.63}         & \multicolumn{1}{c|}{0.61}         & \multicolumn{1}{c|}{0.62}         & \multicolumn{1}{c|}{0.74}         & 0.50                      \\ \hline
\textbf{MKB}                            & \multicolumn{1}{c|}{0.65}          & \multicolumn{1}{c|}{0.65}         & \multicolumn{1}{c|}{0.65}         & \multicolumn{1}{c|}{0.70}         & 0.52                      & \multicolumn{1}{c|}{0.67}         & \multicolumn{1}{c|}{0.64}         & \multicolumn{1}{c|}{0.65}         & \multicolumn{1}{c|}{0.72}         & 0.56                      & \multicolumn{1}{c|}{0.58}          & \multicolumn{1}{c|}{0.58}         & \multicolumn{1}{c|}{0.58}         & \multicolumn{1}{c|}{0.69}         & 0.35                      & \multicolumn{1}{c|}{0.60}         & \multicolumn{1}{c|}{0.59}         & \multicolumn{1}{c|}{0.62}         & \multicolumn{1}{c|}{0.72}         & 0.38                      & \multicolumn{1}{c|}{0.62}          & \multicolumn{1}{c|}{0.62}         & \multicolumn{1}{c|}{0.62}         & \multicolumn{1}{c|}{0.70}         & 0.43                      & \multicolumn{1}{c|}{0.63}         & \multicolumn{1}{c|}{0.61}         & \multicolumn{1}{c|}{0.62}         & \multicolumn{1}{c|}{0.72}         & 0.47                      \\ \hline
\textbf{PM-speech}                      & \multicolumn{1}{c|}{0.70}          & \multicolumn{1}{c|}{0.68}         & \multicolumn{1}{c|}{0.68}         & \multicolumn{1}{c|}{0.74}         & 0.6                       & \multicolumn{1}{c|}{0.68}         & \multicolumn{1}{c|}{0.64}         & \multicolumn{1}{c|}{0.65}         & \multicolumn{1}{c|}{0.73}         & 0.59                      & \multicolumn{1}{c|}{0.60}          & \multicolumn{1}{c|}{0.59}         & \multicolumn{1}{c|}{0.59}         & \multicolumn{1}{c|}{0.71}         & 0.38                      & \multicolumn{1}{c|}{0.60}         & \multicolumn{1}{c|}{0.58}         & \multicolumn{1}{c|}{0.59}         & \multicolumn{1}{c|}{0.74}         & 0.40                      & \multicolumn{1}{c|}{0.64}          & \multicolumn{1}{c|}{0.63}         & \multicolumn{1}{c|}{0.64}         & \multicolumn{1}{c|}{0.72}         & 0.48                      & \multicolumn{1}{c|}{0.64}         & \multicolumn{1}{c|}{0.61}         & \multicolumn{1}{c|}{0.62}         & \multicolumn{1}{c|}{0.74}         & 0.49                      \\ \hline
\textbf{INC}                            & \multicolumn{1}{c|}{0.69}          & \multicolumn{1}{c|}{0.62}         & \multicolumn{1}{c|}{0.62}         & \multicolumn{1}{c|}{0.73}         & 0.62                      & \multicolumn{1}{c|}{0.69}         & \multicolumn{1}{c|}{0.60}         & \multicolumn{1}{c|}{0.60}         & \multicolumn{1}{c|}{0.73}         & 0.63                      & \multicolumn{1}{c|}{0.60}          & \multicolumn{1}{c|}{0.58}         & \multicolumn{1}{c|}{0.58}         & \multicolumn{1}{c|}{0.73}         & 0.39                      & \multicolumn{1}{c|}{0.60}         & \multicolumn{1}{c|}{0.57}         & \multicolumn{1}{c|}{0.57}         & \multicolumn{1}{c|}{0.74}         & 0.40                      & \multicolumn{1}{c|}{0.63}          & \multicolumn{1}{c|}{0.59}         & \multicolumn{1}{c|}{0.60}         & \multicolumn{1}{c|}{0.73}         & 0.48                      & \multicolumn{1}{c|}{0.63}         & \multicolumn{1}{c|}{0.58}         & \multicolumn{1}{c|}{0.60}         & \multicolumn{1}{c|}{0.74}         & 0.49                      \\ \hline
\textbf{PIB}                            & \multicolumn{1}{c|}{0.67}          & \multicolumn{1}{c|}{0.70}         & \multicolumn{1}{c|}{0.68}         & \multicolumn{1}{c|}{0.70}         & 0.51                      & \multicolumn{1}{c|}{0.67}         & \multicolumn{1}{c|}{0.62}         & \multicolumn{1}{c|}{0.60}         & \multicolumn{1}{c|}{0.73}         & 0.57                      & \multicolumn{1}{c|}{0.60}          & \multicolumn{1}{c|}{0.63}         & \multicolumn{1}{c|}{0.60}         & \multicolumn{1}{c|}{0.67}         & 0.36                      & \multicolumn{1}{c|}{0.60}         & \multicolumn{1}{c|}{0.59}         & \multicolumn{1}{c|}{0.59}         & \multicolumn{1}{c|}{0.72}         & 0.38                      & \multicolumn{1}{c|}{0.63}          & \multicolumn{1}{c|}{0.66}         & \multicolumn{1}{c|}{0.64}         & \multicolumn{1}{c|}{0.68}         & 0.43                      & \multicolumn{1}{c|}{0.63}         & \multicolumn{1}{c|}{0.61}         & \multicolumn{1}{c|}{0.62}         & \multicolumn{1}{c|}{0.73}         & 0.47                      \\ \hline
\multicolumn{1}{|l|}{\textbf{Bhaskar}}  & \multicolumn{1}{l|}{0.67}          & \multicolumn{1}{l|}{0.70}         & \multicolumn{1}{l|}{0.67}         & \multicolumn{1}{l|}{0.68}         & \multicolumn{1}{l|}{0.49} & \multicolumn{1}{l|}{0.68}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.54}         & \multicolumn{1}{l|}{0.71}         & \multicolumn{1}{l|}{0.64} & \multicolumn{1}{l|}{0.90}          & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.67}         & \multicolumn{1}{l|}{0.36} & \multicolumn{1}{l|}{0.70}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.78}         & \multicolumn{1}{l|}{0.60} & \multicolumn{1}{l|}{0.64}          & \multicolumn{1}{l|}{0.67}         & \multicolumn{1}{l|}{0.64}         & \multicolumn{1}{l|}{0.67}         & \multicolumn{1}{l|}{0.42} & \multicolumn{1}{l|}{0.70}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.55}         & \multicolumn{1}{l|}{0.75}         & \multicolumn{1}{l|}{0.62} \\ \hline
\multicolumn{1}{|l|}{\textbf{Jagran}}   & \multicolumn{1}{l|}{0.68}          & \multicolumn{1}{l|}{0.59}         & \multicolumn{1}{l|}{0.58}         & \multicolumn{1}{l|}{0.72}         & \multicolumn{1}{l|}{0.63} & \multicolumn{1}{l|}{0.68}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.54}         & \multicolumn{1}{l|}{0.71}         & \multicolumn{1}{l|}{0.65} & \multicolumn{1}{l|}{0.62}          & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.75}         & \multicolumn{1}{l|}{0.44} & \multicolumn{1}{l|}{0.70}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.78}         & \multicolumn{1}{l|}{0.6}  & \multicolumn{1}{l|}{0.65}          & \multicolumn{1}{l|}{0.57}         & \multicolumn{1}{l|}{0.57}         & \multicolumn{1}{l|}{0.74}         & \multicolumn{1}{l|}{0.52} & \multicolumn{1}{l|}{0.69}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.55}         & \multicolumn{1}{l|}{0.75}         & \multicolumn{1}{l|}{0.62} \\ \hline
\multicolumn{1}{|l|}{\textbf{Speech}}   & \multicolumn{1}{l|}{0.67}          & \multicolumn{1}{l|}{0.64}         & \multicolumn{1}{l|}{0.65}         & \multicolumn{1}{l|}{0.72}         & \multicolumn{1}{l|}{0.56} & \multicolumn{1}{l|}{0.67}         & \multicolumn{1}{l|}{0.64}         & \multicolumn{1}{l|}{0.65}         & \multicolumn{1}{l|}{0.72}         & \multicolumn{1}{l|}{0.56} & \multicolumn{1}{l|}{0.60}          & \multicolumn{1}{l|}{0.59}         & \multicolumn{1}{l|}{0.59}         & \multicolumn{1}{l|}{0.72}         & \multicolumn{1}{l|}{0.39} & \multicolumn{1}{l|}{0.60}         & \multicolumn{1}{l|}{0.59}         & \multicolumn{1}{l|}{0.59}         & \multicolumn{1}{l|}{0.72}         & \multicolumn{1}{l|}{0.39} & \multicolumn{1}{l|}{0.63}          & \multicolumn{1}{l|}{0.61}         & \multicolumn{1}{l|}{0.62}         & \multicolumn{1}{l|}{0.72}         & \multicolumn{1}{l|}{0.47} & \multicolumn{1}{l|}{0.63}         & \multicolumn{1}{l|}{0.61}         & \multicolumn{1}{l|}{0.62}         & \multicolumn{1}{l|}{0.72}         & \multicolumn{1}{l|}{0.47} \\ \hline
\multicolumn{1}{|l|}{\textbf{News}}     & \multicolumn{1}{l|}{0.68}          & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.54}         & \multicolumn{1}{l|}{0.71}         & \multicolumn{1}{l|}{0.65} & \multicolumn{1}{l|}{0.68}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.54}         & \multicolumn{1}{l|}{0.71}         & \multicolumn{1}{l|}{0.65} & \multicolumn{1}{l|}{0.71}          & \multicolumn{1}{l|}{0.57}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.78}         & \multicolumn{1}{l|}{0.63} & \multicolumn{1}{l|}{0.71}         & \multicolumn{1}{l|}{0.57}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.78}         & \multicolumn{1}{l|}{0.63} & \multicolumn{1}{l|}{0.70}          & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.55}         & \multicolumn{1}{l|}{0.76}         & \multicolumn{1}{l|}{0.64} & \multicolumn{1}{l|}{0.70}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.55}         & \multicolumn{1}{l|}{0.76}         & \multicolumn{1}{l|}{0.64} \\ \hline
\multicolumn{1}{|l|}{\textbf{Combined}} & \multicolumn{1}{l|}{0.68}          & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.54}         & \multicolumn{1}{l|}{0.71}         & \multicolumn{1}{l|}{0.65} & \multicolumn{1}{l|}{0.68}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.54}         & \multicolumn{1}{l|}{0.71}         & \multicolumn{1}{l|}{0.65} & \multicolumn{1}{l|}{0.70}          & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.78}         & \multicolumn{1}{l|}{0.6}  & \multicolumn{1}{l|}{0.70}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.78}         & \multicolumn{1}{l|}{0.6}  & \multicolumn{1}{l|}{0.69}          & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.55}         & \multicolumn{1}{l|}{0.75}         & \multicolumn{1}{l|}{0.62} & \multicolumn{1}{l|}{0.69}         & \multicolumn{1}{l|}{0.56}         & \multicolumn{1}{l|}{0.55}         & \multicolumn{1}{l|}{0.75}         & \multicolumn{1}{l|}{0.62} \\ \hline
\end{tabular}}
\caption{Temporary table with detailed precision, recall, f-score values, accuracy value, accuracy 2 (if a paragraph is classified code-mixed by our model and the paragraph is actually code-mixed, we add 1 to the score and if it is classified code-mixed and the paragraph is not, we add to the score. The score divided by the total number of Code-mixed paragraph identified is the acc-2) }
\end{table*}

==> tables/parameters.tex <==
\begin{table*}[hbt!]
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Category}       & \textbf{\begin{tabular}[c]{@{}l@{}}Thresh\\(sent)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Thresh\\ (para)\end{tabular}} & \textbf{F-score} & \textbf{Articles} & \textbf{\# Articles} & \textbf{\# Paragraphs} & \textbf{Avg Words} & \textbf{Avg Characters} \\ \hline
\textbf{AAP}            & 25                                                                        & 0.21                                                                  & 0.68             & 5                                      & 307                         & 689                          & 485                          & 2489                              \\ \hline
\textbf{MKB}            & 32                                                                        & 0.35                                                                  & 0.63             & 2                                      & 67                          & 880                          & 213                          & 992                               \\ \hline
\textbf{PM-speech}      & 21                                                                        & 0.4                                                                   & 0.75             & 3                                      & 653                         & 10931                        & 139                          & 660                               \\ \hline
\textbf{President}      & 22                                                                        & 0.22                                                                  & 0.63             & 3                                      & -                           & -                            & -                            & -                                 \\ \hline
\textbf{PIB}            & 29                                                                        & 0.25                                                                  & 0.61             & 50                                     & 9579                        & 19160                        & 278                          & 1514                              \\ \hline
\textbf{Bhaskar}        & 28                                                                        & 0.2                                                                   & 0.62             & 30                                     & 64121                       & 115324                       & 68                           & 329                               \\ \hline
\textbf{Jagran}         & 20                                                                        & 0.27                                                                  & 0.64             & 30                                     & 227606                      & -                            & -                            & -                                 \\ \hline
{\ul \textbf{Combined}} &                                                                           &                                                                       &                  &                                        &                             &                              &                              &                                   \\ \hline
\textbf{News}           & 28                                                                        & 0.2                                                                   & 0.62             & 60                                     & 282856                      & 891264                       & 63                           & 313                               \\ \hline
\textbf{Political}      & 26                                                                        & 0.25                                                                  & 0.63             & 63                                     & 1158                        & 11674                        & 173                          & 840                               \\ \hline
\end{tabular}
\caption{}
\label{tab: parameters}
\end{table*}

==> tables/parameters_new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\resizebox{\hsize}{!}{
\begin{tabular}{l|c|ccc|ccc|ccc|cccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{\textit{\begin{tabular}[c]{@{}c@{}}Source \\Dataset\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textit{Articles}}} & \multicolumn{3}{c|}{\textit{Paragrpahs}}                                       & \multicolumn{3}{c|}{\textit{\begin{tabular}[c]{@{}c@{}}Threshold Search on\\ Source Dataset\end{tabular}}} & 
\multicolumn{3}{c|}{\textit{ELIT}} &
\multicolumn{4}{c}{\textit{MVT}}
\\ 
% \cline{3-14}
\multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{c|}{}                                   & \multicolumn{1}{c}{Total} & \multicolumn{1}{c}{Hing} & \multicolumn{1}{c|}{E/H} & \multicolumn{1}{c}{$A_{SD}$} & \multicolumn{1}{c}{$t_{sent}$} & \multicolumn{1}{c|}{$t_{para}$} & \multicolumn{1}{c}{{$A^E_s$}} & \multicolumn{1}{c}{{$A^E_n$}} & \multicolumn{1}{c|}{{$A^E_{s+n}$}} & \multicolumn{1}{c}{{$A^M_s$}}      & \multicolumn{1}{c}{{$A^M_n$}} & \multicolumn{1}{c}{{$A^M_{s+n}$}}     &
\multicolumn{1}{c}{{$A^M_{SD}$}}
\\ \hline 
AAP &5 & 6 & 2 &4 &1.0 & 25 & 0.35 & 0.72 & 0.72 & 0.73 & 0.73 & 0.74 & 0.74 & 1.0 \\
MKB &3 & 66 & 25 & 41 & 0.64 &22 &0.35 & 0.70 & 0.69 & 0.70 & 0.72 & 0.72 & 0.72 & 0.76\\
PIB & 47 & 62 & 27 &35&0.68&26&0.15 & 0.70 & 0.67 & 0.67 & 0.73 & 0.72 & 0.73 & 0.72\\
PMS & 2 &  36 & 13 & 23 & 0.89 &21   & 0.45 & 0.74 & 0.71 & 0.72  & 0.73 & 0.74 & 0.74 & 0.92\\
INC & 3 & 69 & 5 & 64 & 0.89&28 & 0.3 & 0.73 & 0.73 & 0.73 & 0.73 & 0.74 & 0.74 & 0.89 \\ \hline
DB & 30 & 207 & 48 & 159 & 0.72&18  & 0.4 & 0.68  & 0.67 & 0.67 & 0.71 & 0.78 & 0.75 & 0.75\\
DJ & 30 & 122 & 28 & 94 &0.79&28 &0.4 & 0.72 & 0.75 & 0.74 & 0.71 & 0.78 & 0.75 & 0.87\\ \hline
$D_{speech}$ & 60 & 239 & 72 & 167 & 0.72&24 & 0.35 & 0.72 & 0.72 & 0.72 & 0.72 & 0.72 & 0.72 & 0.72\\ \hline
$D_{news}$ & 60 & 329 & 76 & 253 & 0.78&29 & 0.475 & 0.71 & 0.78 & 0.76 & 0.71 & 0.78 & 0.76 & 0.78 \\ \hline
\begin{tabular}[c]{@{}c@{}}$D_{speech}$ \\ + $D_{news}$\end{tabular} & 120 & 568 & 121 & 420 & 0.75&29 & 0.45 & 0.71 & 0.78 & 0.75 & 0.71 & 0.78 & 0.75 & 0.75\\ \hline
\end{tabular}}
\caption{Identification of code-mixed Hinglish paragraphs using the best threshold search on the gold standard dataset. Articles: number of annotated articles from each dataset. Total: total number of paragraphs. Hing: number of Hinglish paragraphs. E/H: number of monolingual paragraphs. $A_{SD}$: the best-identified accuracy on the annotated source dataset. $A^E_s$, $A^E_n$, and $A^E_{s+n}$: respective accuracy scores on the annotated $D_{speech}$, $D_{news}$, and $D_{speech}$ + $D_{news}$ datasets using the ELIT technique. $A^M_s$, $A^M_n$, and $A^M_{s+n}$: respective accuracy scores on the annotated $D_{speech}$, $D_{news}$, and $D_{speech}$ + $D_{news}$ datasets using the MVT technique. $A^M_{SD}$: Accuracy on the source dataset using the MVT technique.}
\label{tab: parameters}
\end{table*}

==> tables/result_CK.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!tbh]
\resizebox{\hsize}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
\hline
\multirow{2}{*}{\textit{Source}} & \multicolumn{3}{c|}{\textit{LA}} & \multicolumn{3}{c|}{\textit{GA}} & \multicolumn{3}{c|}{\textit{ALG}} & \multicolumn{3}{c|}{\textit{SDG}} & \multicolumn{3}{c}{\textit{MDG}} \\
& $A_n$ & $A_s$ & $A_{s+n}$ & $A_n$ & $A_s$ & $A_{s+n}$ & $A_n$ & $A_s$ & $A_{s+n}$ & $A_n$ & $A_s$ & $A_{s+n}$ & $A_n$ & $A_s$ & $A_{s+n}$  \\ \hline
AAP & 0.16 & 0.02 & 0.06 & 0.18 & 0.14 & 0.19 & 0.18 & 0.04 & 0.10 & 0.28 & 0.10 & 0.20 & 0.28 & 0.14 & 0.20 \\
INC & 0.11 & 0.07 & 0.11 & 0.18 & 0.14 & 0.19 & 0.13 & 0.04 & 0.12 & 0.22 & 0.15 & 0.20 & 0.22 & 0.17 & 0.20 \\
MKB & 0.18 & 0.06 & 0.16 & 0.18 & 0.14 & 0.19 & 0.18 & 0.08 & 0.11 & 0.28 & 0.16 & 0.25 & 0.28 & 0.18 & 0.25 \\
PIB & 0.20 & 0.07 & 0.17 & 0.18 & 0.14 & 0.19 & 0.19 & 0.09 & 0.15 & 0.30 & 0.15 & 0.26 & 0.30 & 0.20 & 0.26 \\
PMS & 0.18 & 0.05 & 0.10 & 0.18 & 0.14 & 0.19 & 0.19 & 0.06 & 0.18 & 0.29 & 0.21 & 0.21 & 0.29 & 0.21 & 0.21 \\
DB  & 0.20 & 0.09 & 0.17 & 0.18 & 0.08 & 0.15 & 0.19 & 0.11 & 0.16 & 0.33 & 0.18 & 0.28 & 0.35 & 0.18 & 0.29 \\
DJ  & 0.17 & 0.06 & 0.15 & 0.18 & 0.08 & 0.15 & 0.20 & 0.13 & 0.15 & 0.27 & 0.11 & 0.13 & 0.29 & 0.11 & 0.14 
\end{tabular}}
\caption{CK}
\label{tab: accuracy_result}
\end{table*}

==> tables/result_MCC.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!tbh]
\resizebox{\hsize}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
\hline
\multirow{2}{*}{\textit{Source}} & \multicolumn{3}{c|}{\textit{LA}} & \multicolumn{3}{c|}{\textit{GA}} & \multicolumn{3}{c|}{\textit{ALG}} & \multicolumn{3}{c|}{\textit{SDG}} & \multicolumn{3}{c}{\textit{MDG}} \\
 & $A_n$ & $A_s$ & $A_{s+n}$ & $A_n$ & $A_s$ & $A_{s+n}$ & $A_n$ & $A_s$ & $A_{s+n}$ & $A_n$ & $A_s$ & $A_{s+n}$ & $A_n$ & $A_s$ & $A_{s+n}$ \\ \hline
AAP & 0.16 & 0.01 & 0.07 & 0.16 & 0.01 & 0.07 & 0.18 & 0.04 & 0.11 & 0.28 & 0.12 & 0.21 & 0.28 & 0.15 & 0.21 \\
INC & 0.11 & 0.08 & 0.12 & 0.11 & 0.08 & 0.12 & 0.13 & 0.05 & 0.12 & 0.22 & 0.16 & 0.21 & 0.22 & 0.20 & 0.21 \\
MKB & 0.19 & 0.06 & 0.16 & 0.19 & 0.06 & 0.16 & 0.18 & 0.08 & 0.12 & 0.28 & 0.16 & 0.25 & 0.28 & 0.18 & 0.25 \\
PIB & 0.20 & 0.07 & 0.17 & 0.20 & 0.07 & 0.17 & 0.19 & 0.09 & 0.15 & 0.31 & 0.15 & 0.26 & 0.31 & 0.19 & 0.26 \\
PMS & 0.18 & 0.02 & 0.11 & 0.18 & 0.02 & 0.11 & 0.20 & 0.07 & 0.18 & 0.29 & 0.22 & 0.21 & 0.29 & 0.22 & 0.21 \\
DB  & 0.21 & 0.09 & 0.17 & 0.21 & 0.09 & 0.17 & 0.19 & 0.12 & 0.16 & 0.35 & 0.18 & 0.28 & 0.37 & 0.18 & 0.29 \\
DJ  & 0.17 & 0.07 & 0.15 & 0.17 & 0.07 & 0.15 & 0.22 & 0.13 & 0.14 & 0.29 & 0.12 & 0.15 & 0.30 & 0.12 & 0.16 
\end{tabular}}
\caption{MCC}
\label{tab: accuracy_result}
\end{table*}

==> tables/result_MUTANT.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!tbh]
\resizebox{\hsize}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
\hline
\multirow{2}{*}{\textit{Source}} & \multicolumn{3}{c|}{\textit{LA}} & \multicolumn{3}{c|}{\textit{GA}} & \multicolumn{3}{c|}{\textit{ALG}} & \multicolumn{3}{c|}{\textit{SDG}} & \multicolumn{3}{c}{\textit{MDG}} \\
 & $A_s$ & $A_n$ & $A_{s+n}$ & $A_s$ & $A_n$ & $A_{s+n}$ & $A_s$ & $A_n$ & $A_{s+n}$ & $A_s$ & $A_n$ & $A_{s+n}$ & $A_s$ & $A_n$ & $A_{s+n}$ \\ \hline
AAP & 72  & 62 & 69 & 70  & 66 & 70 & 71 & 64 & 69 & 72 & 72 & 73 & 73 & 74 & 74 \\
INC & 69 & 63 & 70 & 70 & 66 & 70 & 71 & 64 & 69 & 73 & 73 & 73 & 73 & 74 & 74 \\
MKB & 66 & 61 & 67 & 70 & 66 & 70 & 68 & 62 & 69 & 70 & 69 & 70 & 72 & 72 & 72 \\
PIB & 68 & 62 & 69 & 70 & 66 & 70 & 68 & 64 & 69 & 70 & 67 & 67 & 73 & 72 & 73 \\
PMS & 61 & 67 & 62 & 70 & 66 & 70 & 69 & 64 & 70 & 74 & 71 & 72 & 73 & 74 & 74 \\
DB & 66 & 61 & 67 & 69 & 63 & 68 & 67 & 62 & 67 & 68 & 67 & 67 & 71 & 78 & 75 \\
DJ & 68 & 62 & 68 & 69 & 63 & 68 & 68 & 64 & 69 & 72 & 75 & 74 & 71 & 78 & 75 \\ \hline
\end{tabular}}
\caption{}
\label{tab: accuracy_result}
\end{table*}

==> tables/result_WA.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!tbh]
\resizebox{\hsize}{!}{
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
\hline
\multirow{2}{*}{\textit{Source}} & \multicolumn{3}{c|}{\textit{LA}} & \multicolumn{3}{c|}{\textit{GA}} & \multicolumn{3}{c|}{\textit{ALG}} & \multicolumn{3}{c|}{\textit{SDG}} & \multicolumn{3}{c}{\textit{MDG}} \\
 & $A_n$ & $A_s$ & $A_{s+n}$ & $A_n$ & $A_s$ & $A_{s+n}$ & $A_n$ & $A_s$ & $A_{s+n}$ & $A_n$ & $A_s$ & $A_{s+n}$ & $A_n$ & $A_s$ & $A_{s+n}$ \\ \hline
AAP & 58 & 49 & 64 & 58 & 60 & 58 & 59 & 49 & 56 & 69 & 61 & 66 & 66 & 61 & 66 \\
INC & 56 & 50 & 57 & 58 & 60 & 58 & 56 & 53 & 57 & 63 & 61 & 64 & 69 & 65 & 67 \\
MKB & 58 & 53 & 58 & 58 & 60 & 58 & 57 & 55 & 57 & 64 & 59 & 64 & 66 & 62 & 56 \\
PIB & 59 & 54 & 59 & 58 & 60 & 58 & 59 & 55 & 58 & 55 & 63 & 56 & 64 & 62 & 64 \\
PMS & 59 & 51 & 56 & 58 & 60 & 58 & 59 & 54 & 58 & 65 & 63 & 62 & 65 & 62 & 65 \\
DB  & 59 & 54 & 58 & 60 & 53 & 59 & 59 & 53 & 58 & 71 & 64 & 69 & 74 & 52 & 63 \\
DJ  & 58 & 53 & 57 & 60 & 53 & 59 & 60 & 58 & 59 & 74 & 63 & 64 & 74 & 53 & 64 
\end{tabular}}
\caption{Weighted Average}
\label{tab: accuracy_result}
\end{table*}

==> tables/summ_results.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|ccc}
\hline
\textit{Model} & \textit{R1} & \textit{R2} & \textit{RL} \\ \hline
\textit{T5} & 2.63 & 0.03 & 2.42 \\
\textit{Pegasus} & 5.37  & 0.40   & 1.69 \\
\textit{BART} & 1.69 & 0.40 & 1.69 \\
\textit{mT5} & 1.13 & 0.02 & 0.99 \\
\textit{mT5-CrossSum} & 0.86  & 0.20 & 0.86 \\
\textit{mBART} & 6.72 & 1.04 & 6.72 \\
 \hline
$mBART_{2k}$ & 7.90 & 2.53 & 7.74  \\ \hline
$mBART^{roman}$ &21.93 &7.59 & 16.56\\
$mBART^{roman}_{2k}$ & 22.33  & 7.66  & 16.60  \\ \hline
\end{tabular}
\caption{Abstractive summarization results.}
\label{tab:summ_results}
\end{table}

==> tables/summarization.tex <==
\begin{table}[hbt!]
\resizebox{\hsize}{!}{
\begin{tabular}{l|ccccc}
\hline
\textit{Source}  & \textit{Articles} & \textit{AWS} & \textit{ACS} & \textit{AWA} & \textit{ACS}\\ \hline
AAP & 8 & 17 & 86 & 1103 & 5749  \\ 
PMS & 153 & 18 & 106 & 113 & 577  \\ 
PIB & 3470 & 21 & 122 & 488 & 2793  \\ \hline 
DB & 10226 & 23 & 124 & 90 & 450  \\ 
DJ & 20714 & 18 & 96 & 126 & 647  \\ \hline
$D_{speech}$ & 3631 & 21 & 121 & 474 & 2706  \\ \hline 
$D_{news}$ & 30940 & 20 & 105 & 114 & 582  \\ \hline 
\begin{tabular}[c]{@{}c@{}}$D_{speech}$ \\ + $D_{news}$\end{tabular} & 34571 & 20 & 106 & 151 & 805  \\ \\ \hline  
\end{tabular}}
\caption{Distribution of the dataset for the summarization tasks from various data sources. AWS: average number of words in a summary. ACS: average number of characters in a summary. AWA: average number of words in an article. ACS: average number of words in an article.}
\label{tab: summary_data}
\end{table}

==> tables/tokens.tex <==
\begin{table}[hbt!]
\resizebox{\hsize}{!}{
\begin{tabular}{l|cccc}
\hline
\textbf{Source}          
&\multicolumn{1}{l}{\textbf{Total Tokens}} &\multicolumn{1}{l}{\textbf{\% Hindi}}
&\multicolumn{1}{l}{\textbf{\% English}} 
&\multicolumn{1}{l}{\textbf{\% Other}} \\ \hline
\textbf{AAP} & 357858 & 53.97 & 45.09 & 0.94 \\ \hline
\textbf{MKB} & 273238 & 77.17 & 22.41 & 0.42 \\ \hline
\textbf{PIB} & 15982360 & 80.96 & 17.59 & 1.45 \\ \hline
\textbf{PMS} & 1832295 & 79.02 & 20.45 & 0.53 \\ \hline
\textbf{INC} & 222608 & 63.83 & 33.12 & 3.03 \\ \hline
\textbf{DB} & 46275432 & 80.22 & 18.25 & 1.53 \\ \hline
\textbf{DJ} & 111581201 & 79.28 & 19.60 & 1.12  \\ \hline
\end{tabular}}
\caption{Distribution of the identified languages in each dataset.}
\label{tab: token_percentage}
\end{table}
